\textit{A Posteriori} local subcell correction of high-order discontinuous Galerkin scheme for conservation laws on two-dimensional unstructured grids

We present the two-dimensional unstructured grids extension of the a posteriori local subcell correction of discontinuous Galerkin (DG) schemes introduced in [52]. The technique is based on the reformulation of DG scheme as a finite volume (FV) like method through the definition of some specific numerical fluxes referred to as reconstructed fluxes. High-order DG numerical scheme combined with this new local subcell correction technique ensures positivity preservation of the solution, along with a low oscillatory and sharp shocks representation. The main idea of this correction procedure is to retain as much as possible the high accuracy and the very precise subcell resolution of DG schemes, while ensuring the robustness and stability of the numerical method, as well as preserving physical admissibility of the solution. Consequently, an a posteriori correction will only be applied locally at the subcell scale where it is needed, but still ensuring the local scheme conservation. Practically, at each time step, we compute a DG candidate solution and check if this solution is admissible (for instance positive, non-oscillating, etc). Numerical results on various type problems and test cases will be presented to assess the very good performance of the design correction algorithm.

==> SOURCES/DG.tex <==
\section{Discontinuous Galerkin scheme}
\label{sect_DG}

This section is devoted to the recall of discontinuous Galerkin schemes in the very simple case of a one-dimensional Scalar Conservation Law (SCL). Let $u=u(x,t)$, for $x \in \omega$, where $\omega\subset \mathbb{R}$, and $t \in [0,T]$, be the solution of the following system

\begin{subequations}
\label{lcs_eq1D}
\begin{alignat}{2}[left = \empheqlbrace\,]
&\dt{u}+ \dx{F(u)}=0, \qqquad& (x,t)\in\,\omega\times[0,T], \label{lcs1}\\
&u(x,0)=u^0(x), &x\in\,\omega, \label{lcs2}
\end{alignat}
\end{subequations}

where $u^0$ is the initial data and $F(u)$ is the flux function. For the subsequent discretization, let us introduce the following notation. Let $\{\omega_i\}_i$ be a partition of the computational domain $\omega$. Here, $\omega_i=[x_{\imdemi},x_{\ipdemi}]$ denotes a generic computational cell of size $\Delta x_i$. We also introduce a partition of the time domain $0=t^1 < t^2<... <t^n<... < t^N=T$ and the time step $\Delta t^n=t^{n+1}-t^{n}$. In order to obtain a $(k+1)\thf$ order discretization, let us consider a piecewise polynomial approximated solution $u_h(x,t)$, where its restriction to cell $\omega_i$, namely $u_{h|\omega_i}=u_h^i$, belongs to $\P^k(\omega_i)$ the set of polynomial of degree up to $k$ and then writes

\begin{align}
  \label{uh_1D}
  u_h^i(x,t)=\Sum_{m=1}^{k+1}u_m^i(t)\,\sigma_m(x),
\end{align}

where $\{\sigma_m\}_m$ is a basis of $\P^k(\omega_i)$. The coefficients $u_m^i$ present in \eqref{uh_1D} are the solution moments to be computed through a local variational formulation on $\omega_i$. To this end, one has to multiply equation \eqref{lcs1} by $\psi \in\,\P^k(\omega_i)$, a polynomial test function, and integrate it on $\omega_i$ as follows

\begin{align*}
  \Int_{\omega_i} \(\dt{u}+\dx{F(u)}\)\psi\,\dd x=0.
\end{align*}

By means of an integration by parts, one gets

\begin{align*}
\Int_{\omega_i} \dt{u}\psi\,\dd x-\Int_{\omega_i} F(u)\dx{\psi}\,\dd x+\Big[F(u)\,\psi\Big]_{x_\im}^{x_\ip}=0.
\end{align*}

We then substitute the solution $u$ by its approximated polynomial counterpart $u_h^i$. And because the numerical solution is assumed to be piecewise continuous, to ensure the scheme conservation we introduce at the cell boundaries $x_{\ipmdemi}$ some flux function $\mc{F}_{\ipmdemi}$ continuous from one cell to another, namely the numerical flux. Consequently, the DG numerical solution will be the function solution of the following problem

\begin{align}
  \label{DG_1D_1}
  \Int_{\omega_i} \dt{u_h^i}\,\psi\,\dd x=\Int_{\omega_i} F(u_h^i)\dx{\psi}\,\dd x-\Big[\mc{F}\,\psi\Big]_{x_\im}^{x_\ip},\qquad \forall \,\psi\in\P^k(\omega_i).
\end{align}

If the test function $\psi$ is taken among the basis functions, one ends up with the following linear system to solve to obtain the numerical solution coefficients $u_m^i$

\begin{align}
  \label{DG_1D_2}
  \Sum_{m=1}^{k+1}\dt{u_m^i}\,\Int_{\omega_i} \sigma_m\,\sigma_p\,\dd x=\Int_{\omega_i} F(u_h^i)\dx{\sigma_p}\,\dd x-\Big[\mc{F}\,\sigma_p\Big]_{x_\im}^{x_\ip},\qquad \text{for } p=1,\dots,k+1.
\end{align}

In this equation, we recognize $\int_{\omega_i} \sigma_m\,\sigma_p\,\dd x$ the mass matrix coefficient, $\int_{\omega_i} F(u_h^i)\dx{\sigma_p}\,\dd x$ the volume integral and $[\mc{F}\,\sigma_p]_{x_\im}^{x_\ip}$ the surface integral.\\

In \eqref{DG_1D_2}, the numerical flux function $\mc{F}$, in addition to ensure the scheme conservation, is the cornerstone of any finite volume or DG scheme regarding fundamental considerations as stability, positivity and entropy among others. In the context of DG schemes, this numerical flux is defined as a function of the two states on the left and right of each interface, $i.e.$ $\mc{F}_\ip=\mc{F}\(u_h^i(x_\ip,t),u_h^{i+1}(x_\ip,t)\)$. This function is generally obtained through the resolution of an exact or approximated Riemann problem at each interface. For instance, a wide range of numerical fluxes can be put in the following viscous form 

\begin{align}
  \label{num_flux}
  \mc{F}(u,v)=\Frac{F(u)+F(v)}{2}-\Frac{\gamma(u,v)}{2}\,(v-u),
\end{align}

where $\gamma(u,v)>0$ is referred to as the viscosity coefficient and is responsible of the numerical diffusion and hence the stability of the numerical scheme. In the remainder of this paper, to remain as simple as possible, we make use of the very well-known local Lax-Friedrichs numerical flux for which $\gamma(u,v)=\max(|F'(u)|,|F'(v)|)$.\\


==> SOURCES/annex.tex <==
\section{Subresolution basis functions and correction coefficients}
\label{sect_subres_basis}

This appendix aims at giving further details related to the subresolution basis functions and the correction coefficients. First, let us introduce the following change of variable

\begin{alignat*}{3}
  &[0,1] \quad &\longrightarrow \quad &\omega_i=[x_\im,x_\ip],\\
  &\xi \quad  &\longrightarrow \quad &x=x_\im+\xi\,(x_\ip-x_\im).
\end{alignat*}

Let then set $\phi_m(x(\xi))=\varphi_m(\xi)=\sum_{p=0}^k a_p^{(m)}\,\xi^p$, such that

\begin{align*}
\Int_0^1 \varphi_m\,\xi^j\,\dd \xi=\Int_{\wt{\xi}_{m-1}}^{\wt{\xi}_m} \xi^j\,\dd\xi,\qquad \text{for }\; j=0,\dots,k.
\end{align*}

These $k+1$ equations lead to the linear system $\Mat{H}\,\bs{C}^{(m)}=\Mat{\Lambda}\,\bs{D}^{(m)}$, where $\Mat{H}$ is an Hilbert matrix, $\bs{C}^{(m)}$ is the vector containing the $a_p^{(m)}$ coefficients, $\Mat{\Lambda}$ is the diagonal matrix such that $\Mat{\Lambda}_{jj}=\inv{j}$ and $\bs{D}^{(m)}$ is defined as follows

\begin{align*}
  \bs{D}^{(m)}=\begin{pmatrix}
  \wt{\xi}_m-\wt{\xi}_{m-1}\\(\wt{\xi}_m)^2-(\wt{\xi}_{m-1})^2\\\vdots\\(\wt{\xi}_m)^{k+1}-(\wt{\xi}_{m-1})^{k+1}
  \end{pmatrix}.
\end{align*}

Recalling that Hilbert matrices are symmetric, hence also $\Mat{H}^{-1}$ is. The subresolution basis functions finally read as follows 

\begin{align}
  \label{subres_def}
  \varphi_m(\xi)=\bs{D}^{(m)}\pds\Mat{\Lambda}\Mat{H}^{-1}\begin{pmatrix}1\\\xi\\\vdots\\\xi^k\end{pmatrix}.
\end{align}

Let us note that the expression of the inverse of an Hilbert matrix is quite complex. However, recalling the correction coefficients definition

\begin{align*}
  C_\im^{(m)}=\Sum_{p=m+1}^{k+1}\varphi_p(0) \qquad \text{and} \qquad C_\ip^{(m)}=\Sum_{p=1}^m\varphi_p(1),
\end{align*}

one can see that only the subresolution functions values in zero and one are needed. Moreover, if we consider a symmetric distribution of the flux points around the cell center, $i.e.$ $\xi_p=1- \xi_{k+1-p}$, for $p=0,\dots,k+1$, it is then easy to understand only $\varphi_p(0)$ is required, as $\varphi_p(1)=\varphi_{k+2-p}(0)$, for $p=1,\dots,k+1$. It also implies that $C_\ip^{(m)}=C_\im^{(k+1-m)}$, for $m=0,\dots,k+1$. In the end, the correction coefficients can be put into the following expression

\begin{align}
  \label{subres_1}
  C_\im^{(m)}=\(\Sum_{p=m+1}^{k+1} \bs{D}^{(m)}\)\pds \Mat{\Lambda}\Mat{H}^{-1}\begin{pmatrix}1\\0\\\vdots\\0\end{pmatrix}.
\end{align}

Consequently, in regards to equation \eqref{subres_1}, only the first column of $\Mat{H}^{-1}$ is needed. By introducing the vector $\bs{B}=\Mat{\Lambda}\Mat{H}^{-1}\(1,0,\dots,0\)\tra$, and noting that $\bs{B}\pds\(1,\dots,1\)\tra=1$, one gets the following very simple expression of $C_\im^{(m)}$

\begin{align*}
  C_\im^{(m)}=1-\begin{pmatrix}\widetilde{\xi}_m\\(\widetilde{\xi}_m)^2\\\vdots\\(\widetilde{\xi}_m)^{k+1}\end{pmatrix}\pds \bs{B}.
\end{align*}


==> SOURCES/command.tex <==
\newcommand{\id}{\Mat{I}_d}
\newcommand{\dc}{\centerdot}
\newcommand{\fs}[1]{\mathsf{#1}}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\C}{\mathbb C}
\newcommand{\Q}{\mathbb Q}
\newcommand{\K}{\mathbb K}
\def\P{{\mathbb P}}
\def\I{{\mathbb I}}
\def\t{\text{t}}
\def\1{{\mathbbm 1}}

\def\J{{|\Mat{J}|}}

\newcommand{\dpar}[2]{\dfrac{\partial #1}{\partial #2}}
\newcommand{\tpar}[2]{\tfrac{\partial #1}{\partial #2}}
\newcommand{\dd}{\mathrm{d}}
\renewcommand{\d}[2]{\frac{\dd #1}{\dd #2}}
\newcommand{\A}{{\mathcal{ A}}}
\newcommand{\BB}{{\mathcal{ B}}}
\newcommand{\CC}{{\mathcal{ C}}}
\newcommand{\DD}{{\mathcal{ D}}}
\newcommand{\EE}{{\mathcal{ E}}}
\newcommand{\E}{{\mathcal{ E}}}
\newcommand{\FF}{{\mathcal{ F}}}
\newcommand{\GG}{{\mathcal{ G}}}
\newcommand{\Hhh}{{\mathcal{ H}}}
\newcommand{\II}{{\mathcal{ I}}}
\newcommand{\JJ}{{\mathcal{ J}}}
\newcommand{\KK}{{\mathcal{ K}}}
\newcommand{\LL}{{\mathcal{ L}}}
\newcommand{\MM}{{\mathcal{ M}}}
\newcommand{\NN}{{\mathcal{ N}}}
\newcommand{\OO}{{\mathcal{ O}}}
\newcommand{\PP}{{\mathcal{ P}}}
\newcommand{\QQ}{{\mathcal{ Q}}}
\newcommand{\RR}{{\mathcal{ R}}}
\newcommand{\SSS}{{\mathcal{ S}}}
\newcommand{\TT}{{\mathcal{ T}}}
\newcommand{\UU}{{\mathcal{ U}}}
\newcommand{\VV}{{\mathcal{ V}}}
\newcommand{\WW}{{\mathcal{ W}}}
\newcommand{\XX}{{\mathcal{ X}}}
\newcommand{\YY}{{\mathcal{ Y}}}
\newcommand{\ZZ}{{\mathcal{ Z}}}
\newcommand{\dlim}[1]{\displaystyle{\lim _{#1}}}
\newcommand{\dsum}[2]{\displaystyle{\sum _{#1}^{#2}}}
\newcommand{\dprod}[1]{\displaystyle{\prod _{#1}}}
\newcommand{\norm}[1]{\left | \left | #1 \right | \right |}
\newcommand{\abs}[1]{\left | #1 \right |}
\newtheorem{theoreme}{Theorem}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theoreme]{Proposition}
\newtheorem{lemme}[theoreme]{Lemma}
\newtheorem{corollar}[theoreme]{Corollary}
\newtheorem{corollaire}[theoreme]{Corollary}
\newtheorem{remarque}[theoreme]{Remarque}
\newtheorem{remark}[theoreme]{Remark}
\newtheorem{exemple}[theoreme]{Exemple}
\newtheorem{definition}[theoreme]{D\'efinition}
\newtheorem{hypothese}[theorem]{Assumption}
%

\newcommand{\Min}{\displaystyle\min}
\newcommand{\Max}{\displaystyle\max}
\newcommand{\Sup}{\displaystyle\sup}
\newcommand{\mnx}{{\min\backslash\max}}
\newcommand{\xory}{{x\backslash y}}
\newcommand{\Int}{\displaystyle\int}
\newcommand{\Sum}{\displaystyle\sum}
\newcommand{\Lim}[2]{\displaystyle\lim\limits_{#1\,\rightarrow\, #2}}
\newcommand{\Frac}{\displaystyle\frac}
\newcommand{\Bigcup}{\displaystyle\bigcup}
\newcommand{\ov}{\overline}
\newcommand{\un}{\underline}
\newcommand{\wt}{\widetilde}
\newcommand{\bnabla}{\bs{\nabla}}
\newcommand{\minmod}{\text{minmod}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\swh}[1]{\displaystyle\widehat{#1}}
\newcommand{\whc}[1]{\<{#1}\>_c}
\newcommand{\acos}{\text{acos}}
\newcommand{\tr}{\text{tr}}
\newcommand{\tra}{^{\text{t}}}
\newcommand{\thf}{^{\text{th}}}
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\lh}{\hspace*{-2mm}}

\newcommand{\pds}{\centerdot}
\newcommand{\demi}{\frac{1}{2}}
\newcommand{\im}{{i-\demi}}
\newcommand{\ip}{{i+\demi}}
\newcommand{\ipm}{{i\pm\demi}}
\newcommand{\jm}{{j-\demi}}
\newcommand{\jp}{{j+\demi}}
\newcommand{\jpm}{{j\pm\demi}}
\newcommand{\imdemi}{i-\demi}
\newcommand{\ipdemi}{i+\demi}
\newcommand{\jmdemi}{j-\demi}
\newcommand{\jpdemi}{j+\demi}
\newcommand{\ipmdemi}{i\pm\demi}
\newcommand{\impdemi}{i\mp\demi}
\newcommand{\Dt}{\Delta t}
\newcommand{\Dx}{\Delta x}
\newcommand{\DX}{\Delta X}
\newcommand{\DDx}{\nabla_x}
\newcommand{\DDX}{\nabla_X}
\newcommand{\gradx}[1]{\nabla_x{#1}}
\newcommand{\gradX}[1]{\nabla_X{#1}}
\newcommand{\divf}{\nabla\pds}
\newcommand{\divx}{\nabla_x\pds}
\newcommand{\divX}{\nabla_X\pds}
\newcommand{\sdt}[1]{\frac{\partial {\,#1}}{\partial t}}
\newcommand{\dt}[1]{\Frac{\partial {\,#1}}{\partial t}}
\newcommand{\dm}[1]{\Frac{\partial {\,#1}}{\partial m}}
\newcommand{\sdX}[1]{\frac{\partial {\,#1}}{\partial X}}
\newcommand{\dX}[1]{\Frac{\partial {\,#1}}{\partial X}}
\newcommand{\sdx}[1]{\frac{\partial {\,#1}}{\partial x}}
\newcommand{\dx}[1]{\Frac{\partial {\,#1}}{\partial x}}
\newcommand{\dY}[1]{\Frac{\partial {\,#1}}{\partial Y}}
\newcommand{\dy}[1]{\Frac{\partial {\,#1}}{\partial y}}
\newcommand{\sddt}[1]{\frac{\mathrm{d} {\,#1}}{\mathrm{d} t}}
\newcommand{\ddt}[1]{\Frac{\mathrm{d} {\,#1}}{\mathrm{d} t}}
\newcommand{\ddX}[1]{\Frac{\mathrm{d} {\,#1}}{\mathrm{d} X}}
\newcommand{\sddx}[1]{\frac{\mathrm{d} {\,#1}}{\mathrm{d} x}}
\newcommand{\ddx}[1]{\Frac{\mathrm{d} {\,#1}}{\mathrm{d} x}}
\newcommand{\dr}[1]{\Frac{\partial {\,#1}}{\partial r}}
\newcommand{\sdr}[1]{\frac{\partial {\,#1}}{\partial r}}
\newcommand{\ddr}[1]{\Frac{\dd {\,#1}}{\dd r}}
\newcommand{\sddr}[1]{\frac{\dd {\,#1}}{\dd r}}
\newcommand{\dth}[1]{\Frac{\partial {\,#1}}{\partial \theta}}
\newcommand{\sdth}[1]{\frac{\partial {\,#1}}{\partial \theta}}
\newcommand{\ddth}[1]{\Frac{\dd {\,#1}}{\dd \theta}}
\newcommand{\sddth}[1]{\frac{\dd {\,#1}}{\dd \theta}}
\newcommand{\dz}[1]{\Frac{\partial {\,#1}}{\partial z}}
\newcommand{\sdz}[1]{\frac{\partial {\,#1}}{\partial z}}
\newcommand{\vdt}{\partial_t}
\newcommand{\vdx}{\partial_x}
\newcommand{\vdxx}{\partial_{xx}}
\newcommand{\vdy}{\partial_y}
\newcommand{\vdyy}{\partial_{yy}}


\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}

\newcommand{\Mat}[1]{\mathsf{#1}}
\newcommand{\inv}[1]{\frac{1}{#1}}
\newcommand{\Inv}[1]{\Frac{1}{#1}}
\newcommand{\sstar}{_{\star}}
\newcommand{\istar}{^{\star}}
\newcommand{\istart}{^{\star^{\scriptstyle{t}}}}
\newcommand{\bk}[1]{\llbracket{#1}\rrbracket}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\bsmat}[1]{\bs{\Mat{#1}}}
\newcommand{\tm}{\text{-}}
\newcommand{\irho}{\inv{\rho}}
\newcommand{\Irho}{\Inv{\rho}}
\newcommand{\udl}[1]{\underline{#1}}
\newcommand{\bld}[1]{\textbf{#1}}
\newcommand{\wb}[1]{\widebreve{#1}}

\def\veps{\varepsilon}
\def\vphi{\varphi}
\def\<{\left<}%\displaystyle\langle}}
\def\>{\right>}%\displaystyle\rangle}}
\def\({\left(}
\def\){\right)}
%\def\[{\left[}
%\def\]{\right]}

\makeatletter
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
     \mathop{\vbox{\m@th\ialign{##\crcr
\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
                    $\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
  \hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}
\makeatletter

\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\Black}[1]{\textcolor{black}{#1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Gray}[1]{\textcolor{gray}{#1}}
\definecolor{dark-gray}{gray}{0.35}
\newcommand{\Dgray}[1]{\textcolor{dark-gray}{#1}}


\newtheorem{com}{Comment}


\newcommand{\jaumanntau}{\stackrel{\scriptscriptstyle \triangledown}
                                                   {\mbox{$\mathsf{T}$}}}
\newcommand{\truesdelltau}{\stackrel{\scriptscriptstyle \square}}

\setlength{\parindent}{0cm}

